Controllable and Diverse Text Generation in E-commerce

In E-commerce, a key challenge in text generation is to find a good trade-off between word diversity and accuracy (relevance) in order to make generated text appear more natural and human-like. In order to improve the relevance of generated results, conditional text generators were developed that use input keywords or attributes to produce the corresponding text. Prior work, however, do not finely control the diversity of automatically generated sentences. For example, it does not control the order of keywords to put more relevant ones first. Moreover, it does not explicitly control the balance between diversity and accuracy. To remedy these problems, we propose a fine-grained controllable generative model, called~\textit{Apex}, that uses an algorithm borrowed from automatic control (namely, a variant of the \textit{proportional, integral, and derivative (PID) controller}) to precisely manipulate the diversity/accuracy trade-off of generated text. The algorithm is injected into a Conditional Variational Autoencoder (CVAE), allowing \textit{Apex} to control both (i) the order of keywords in the generated sentences (conditioned on the input keywords and their order), and (ii) the trade-off between diversity and accuracy. Evaluation results on real-world datasets show that the proposed method outperforms existing generative models in terms of diversity and relevance. Apex is currently deployed to generate production descriptions and item recommendation reasons in Taobao owned by Alibaba, the largest E-commerce platform in China. The A/B production test results show that our method improves click-through rate (CTR) by 13.17\% compared to the existing method for production descriptions. For item recommendation reason, it is able to increase CTR by 6.89\% and 1.42\% compared to user reviews and top-K item recommendation without reviews, respectively.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> back.evaluation.tex <==
\section{Evaluation}
\label{sec:evaluate}
We evaluate the performance of \textit{Apex} on a real-world dataset. We first verify that the PI controller can totally avert KL vanishing. Then, we compare the performance of \textit{Apex} with baselines using automatic evaluation and human evaluation. We also implement online A/B testing to show the good performance of the proposed \textit{Apex}. Finally, we do a case study to show that our approach can generate text that obeys the order of keywords given by user input.

\subsection{Datasets}
We collect a real world dataset of item descriptions and keywords from the Chinese E-commerce platform, Taobao. This dataset contains $617,181$ items and $927,670$ item text descriptions. Each item description is written by multiple human writers who help sellers write text to attract more customers. According to our statistics, each item on average has about $1.4$ descriptions written by humans and the average number of words in each description is $61.3$. In addition, there are about $14.75$ keywords per item on average. The total size of the vocabulary used is $88,156$. 
% In our task, we generate diverse text based on the given keywords of items and their order, such as cheap (1) and red (2).


\subsection{Baselines}
We compare the performance of \textit{Apex} with the following baselines:
\begin{itemize}[leftmargin=*]
\item Apex-cost: This method uses cost annealing method instead of PI controller for \textit{Apex}.
\item Apex-cyclical: This method uses cyclical annealing method instead of PI controller for \textit{Apex}.
\item Seq2seq~\citep{duvsek2016sequence}: This is the seq2seq model with a maximum likelihood estimator~\citep{sutskever2014sequence}. This paper adopts the Transformer model instead of LSTM in the encoder and decoder for a fair comparison.
\item DP-GAN~\citep{xu2018diversity}: This conditional generator builds on the seqGAN, which uses the first sentence as conditional input.
\item ExpansionNet~\citep{ni2018personalized}: This model conditions on some aspects or keywords of items and user identity to generate personalized and diverse text.
\end{itemize}


\subsection{Experimental Settings}
We implement our experiments using Tensorflow through the Texar platform~\citep{hu2018texar}. We use a three-layer Transformer with default eight heads in the encoder and decoder. While transformer design often includes up to six layers, we find that three are sufficient for our purposes and use that number to improve efficiency. Besides, we adopt three-layer fully connected network with hidden size of $400$, $200$ and $100$ to learn the distribution of latent features. In our experiment, we use 80\%, 10\% and 10\% of the above dataset as the training, validation and testing data. We set the maximum number of words for each reference text to 100. The maximum number of input keywords is $50$. In addition, we set both the dimension of word embedding and order embedding to $512$. The learning rate is set to $0.0001$ with the exponential decay by a decay factor 0.9 every $1000$ training steps. Also, we set the batch size to $100$ for model training. Based on empirical PID tuning rules~\citep{silva2003stability}, we set the coefficient of PI algorithm, $K_p$ and $K_i$, to $-0.01$ and $-0.0001$, respectively. The sampling period, $T_s$, is set to 1 for our PI controller.


% \subsection{Metrics}
% \label{sec:metric}
% Following the prior work~\citep{xu2018diversity,ni2018personalized}, we use following commonly used metrics in NLP to evaluate the performance of different text generators.
% \begin{itemize}[leftmargin=*]
% \item Dis-$n$: This metric denotes the number of distinct $n$-gram, which is used to measure the diversity of generated text.
% \item ROUGE-L~\cite{hovy2006automated}: It is used to measure the Longest Common Subsequence (LCS) for sentence similarity
% \item METEOR~\cite{banerjee2005meteor}: This metric measures the harmonic mean of unigram precision and recall for generated text.
% \item Self-BLEU~\cite{zhu2018texygen}: It is used to measure the diversity of generated text.
% \end{itemize}

%%%%
\begin{figure*}[!t]
  \centering
  \subfigure[KL divergence]{
  \includegraphics[width = 0.43\textwidth]{figure/KL.eps}}
  \hskip -1ex
  \subfigure[Weight.]{
  \includegraphics[width =0.43\textwidth]{figure/weight.eps}}
  \vskip -0.15in
  \caption{(a) illustrates comparison of KL divergence for different methods. We can observe that both cost annealing and cyclical annealing suffer from KL vanishing problem, while our \textit{Apex} totally averts KL vanishing. (b) Weight varies with the training step.}
  \label{fig:KL_vanish}
\end{figure*}


%%% table
\begin{table*}[!thb]
\centering
\caption{Performance comparison for different methods using automatic metrics averaged over 5 random seeds. For Dis-$n$, ROUGE-L, METEOR: higher is better. Self-BLEU: lower is better. }
\begin{tabular}{ |l|c|c|c|c|c|c|c|c|}
 \hline
 Models & Dis-1 & Dis-2 &  Dis-3 & ROUGE-L & METEOR & self-BLEU-1 & self-BLEU-2 & self-BLEU-3 \\
 \hline
Apex-PI-5 &  \textbf{9.266K} & \textbf{127.51K} & \textbf{493.57K} & 0.2354 & \textbf{0.2593} & 0.9857 & 0.9471 & 0.8747 \\
Apex-PI-2 & 9.227K & 125.66K & 477.63K & 0.2358 & 0.2494 & \textbf{0.9841} & \textbf{0.9437} & \textbf{0.8674} \\
Apex-PI-1 & 9.108K & 125.39K & 476.40K & \textbf{0.2364} & 0.2538 & 0.9849 & 0.9454 & 0.8715\\
Apex-cost & 8.904K & 121.06K & 456.57K & 0.2344 & 0.2482  & 0.9853 & 0.9459  & 0.8719 \\
Apex-cyclical & 8.915K & 121.82K & 460.24K  & 0.2347 & 0.2486 & 0.9849 & 0.9444 & 0.8690 \\
Seq2seq & 8.648K & 112.31K & 427.22K & 0.2087  & 0.2399 & 0.9819 & 0.9480 & 0.8776 \\
ExpansionNet & 9.018K & 114.96K & 473.28K &  0.1951 & 0.1822 &0.9854& 0.9442 & 0.8700 \\
DP-GAN  & 8.124K & 102.18K & 413.78K & 0.1920 & 0.1949 & 0.9946 & 0.9849 & 0.9698 \\
\hline
\end{tabular}\label{tab:compare}
\end{table*}


\subsection{PI algorithm for KL vanishing}
We first conduct an experiment to demonstrate that the proposed PI algorithm (a variant of PID) can totally avert the KL vanishing. We compare it with the two representative approaches below:
\begin{itemize}[leftmargin=*]
\item Cost annealing~\citep{bowman2015generating}: This method firstly sets the weight of KL divergence term to 0 in the early stage, and then gradually increases it to $1$ using Sigmoid.
\item Cyclical annealing~\citep{liu2019cyclical}: This method splits the training process into $M$ (e.g., $5$) cycles and each increases the weight from 0 until to 1 using the linear function.
\end{itemize}

Fig.~\ref{fig:KL_vanish} illustrates that the KL divergence and its weight $w$ vary with the training steps for different methods. Note that, here PI-$v$ means we set the KL divergence to a desired value $v$ (e.g., 2) for our designed PI algorithm. We can observe from Fig.~\ref{fig:KL_vanish}(a) that when the training step is close to $100$, the KL divergence of CVAEs gradually decreases to $0$, which means the model suffers from KL vanishing. At that point, our PI algorithm automatically sets the weight to a small value to boost the KL divergence as shown in Fig.~\ref{fig:KL_vanish}(b). After $10,000$ training steps, the PI controller stabilizes the KL divergence at the customized set points, such as $1$, $2$ and $5$. Most importantly, we do not need to tune the PI parameters again for different set points of KL divergence in our experiment.

For the cost annealing method, we use two different hyper-parameters, $9000$ and $18000$, in the sigmoid function~\citep{bowman2015generating} to gradually increase the weight from $0$ until to $1$, as shown in Fig.~\ref{fig:KL_vanish}(b). From~\ref{fig:KL_vanish}(a), we can see that it does not suffer from KL vanishing problem at the beginning of training, because its weight is set to a small value in Fig.~\ref{fig:KL_vanish}(b). However, it gradually suffers from KL vanishing after increasing weight from 0 to 1.

For cyclical annealing, we also use different hyper-parameters (e.g., $5$ and $10$) about the number of cycles to do experiments. We discover that cyclical annealing suffers from KL vanishing a lot, because it blindly changes its weight without using the feedback of KL divergence. In Fig.~\ref{fig:KL_vanish}, it can be seen that when the KL divergence is decreasing at some points, its weight still increases, accelerating KL vanishing.


\subsection{Performance Comparison}
Next, we compare the performance of~\textit{Apex} with the baselines above, as shown in Table~\ref{tab:compare}. We adopt the commonly used metrics in NLP: Dis-$n$~\citep{xu2018diversity}, ROUGE-L~\cite{hovy2006automated}, METEOR~\cite{banerjee2005meteor}, and Self-BLEU~\cite{zhu2018texygen}, to evaluate their performance. Here \textit{Apex-PI-v} represents \textit{Apex} with PI algorithm to control the KL divergence to a desired value, such as $5$, $2$ and $1$. Besides, \textit{Apex-cost-anneal} and \textit{Apex-cyclical-anneal} represent our model but replace the PI algorithm with cost annealing and cyclical annealing to generate text, respectively. Table~\ref{tab:compare} illustrates that \textit{Apex} with PI controller has higher Dis-1, Dis-2 and Dis-3 but lower self-BLEU than the baselines. It means our \textit{Apex} can generate more diverse text than other methods. We also discover that the higher the KL divergence, the more diverse the generated text is. In addition, \textit{Apex} with PI algorithm has higher METEOR and ROUGE-L than the baselines, which means our method can generate relevant text based on keywords. Therefore, the proposed method can achieve a good trade-off between relevance and diversity using PI control algorithm.

\subsection{Accuracy on Controlling Order of Keywords}
We then compare the accuracy in the control of order of keywords for different methods, as shown in Table~\ref{tab:control-accy}. The proposed \textit{Apex} achieves about 97\% accuracy for controlling the order of keywords in the generated sentences. The accuracy for seq2seq, DP-GAN and ExpansionNet, are 40\%, 16\% and 15\%, respectively. Thus, our method significantly outperforms the baseline methods in the control of order of keywords.

%%%%%table below--
\begin{table}[!htb]
\centering
\caption{Controllable accuracy for the order of keywords.}
\vskip -0.1in
\begin{tabular}{|c|c|c|c|}
\hline
Apex & seq2seq & DP-GAN & ExpansionNet \\
\hline
97\% & 40\% & 16\% & 15\% \\
\hline
\end{tabular}\label{tab:control-accy}
\end{table}

\subsection{Expert Post-Editing}
In order to measure the effectiveness of \textit{Apex}, we also ask domain expert to edit the generated sentences until they are fluent, relevant and complete. We randomly select $100$ generated data by \textit{Apex} to conduct experiments. Table~\ref{tab:expert} illustrates the evaluation results  by comparing the generated text before and after expert editing using BLEU, ROUGE and TER scores~\cite{wang2020paperrobot}. We can observe that \textit{Apex} has higher BLEU and ROUGE score and lower TER score than the baselines, which means \textit{Apex} is able to generate high-quality sentences.


\begin{table}[!htb]\footnotesize
\centering
\caption{Evaluation on expert post-editing.}
\vskip -0.1in
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Model & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE & TER \\
\hline
\textit{Apex} & \textbf{0.855} & \textbf{0.837} & \textbf{0.820} & \textbf{0.803} & \textbf{0.898} & \textbf{0.157} \\
\hline
Expans.Net & 0.694 & 0.668 & 0.642 & 0.620 & 0.831 & 0.317 \\
\hline
seq2seq & 0.811 & 0.761 & 0.713 & 0.670 & 0.849 & 0.206 \\
\hline
DP-GAN & 0.647 & 0.628 & 0.609 & 0.593 & 0.828 & 0.371 \\
\hline
\end{tabular}\label{tab:expert}
\end{table}

%%%%
% \begin{table}[!htb]\small
% \centering
% \caption{Evaluation on expert post-editing.}
% \vskip -0.1in
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Model & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE & TER \\
% \hline
% \textit{Apex} & 0.837 & 0.820 & 0.803 & 0.898 & 0.157 \\
% \hline
% ExpansionNet & 0.668 & 0.642 & 0.620 & 0.8307 & 0.317 \\
% \hline
% seq2seq & 0.761 & 0.713 & 0.670 & 0.849 & 0.247 \\
% \hline
% DP-GAN & 0.628 & 0.609 & 0.593 & 0.878 & 0.371 \\
% \hline
% \end{tabular}\label{tab:expert}
% \end{table}

%%%%begin figure
\begin{figure*}[!t]
\centering
\includegraphics[width=0.98\textwidth]{figure/example.pdf}
\caption{Some examples of generated text for item recommendation in Taobao E-commerce platform. Production description is in blue color while recommendation reason is in darkgray color}
\vspace{-0.1 in}
\label{fig:example}
\end{figure*}

\subsection{Online A/B Testing}
We also do A/B test experiments to evaluate the performance of the proposed \textit{Apex}. We deploy \textit{Apex} in a real-world product in Taobao E-commerce platform for two applications: product description generation and item recommendation reason. For each item, we randomly choose one or two from some keywords with an average of 4 to generate different product descriptions and recommendation reasons. To get reliable and convincing evaluation results, the A/B test lasted for one week, from Aug.22th to Aug.28th, 2020. Fig.~\ref{fig:KL_vanish} illustrates some examples of generated text for item recommendation in Taobao. In the first A/B test experiment, we use \textit{Apex} to generate short production descriptions for recommended items, and then compare it with the long production descriptions by the existing method. The A/B test results show that \textit{Apex} can improve the Click-Though Rate (CTR) by 13.17\%. We also get the statistics about user demographics who are more likely to click, and the results show that our text generator improves CTR by 14.9\%, 10.9\% for older people and young people, respectively. For the second application, the proposed method generates one sentence to describe the advantages of the recommended items, and then compare it with user reviews and top-K items without reviews. The test result demonstrates that \textit{Apex} can achieve an improvement of about 6.89\% and 1.42\% in term of CTR over the baseline methods respectively. Therefore, the test experiments further verify the effectiveness of the proposed method.

\subsection{Human Evaluation}
\label{sec:human}
%%%%%---human evaluation---
We ask $25$ human graders to evaluate the relevance and fluency of generated sentences by different methods above. Specifically, we randomly sampled $200$ item text descriptions from each method identically, and mixed (shuffled) them together without telling graders which method generates which text. Then we provided the graders with the input keywords of items, ground truth and the corresponding generated results. The graders were asked to grade relevance and fluency separately on a three point scale based on the our instructions with demo examples. Score ``2'' means the generated text is relevant/fluent, and score ``1'' means it is somewhat relevant/fluent, while score ``0'' means it is not. To ensure the consistency of graders, we computed the Kendall’s tau coefficient to measure the correlation among the graders. The computed score is $0.82$, which indicates high consistency among graders. In addition, we use the two-tailed t-test to compare the scores of our proposed Apex-PI and the baselines. The evaluation results are statistically significant with $p < 0.05$.

%%%%%table below--
\begin{table}[!hbt]\small
\centering
\caption{Scores of fluency and relevance by graders.}
\vskip -0.1in
\begin{tabular}{|l|c|c|c|}
 \hline
 Model & Fluency &Relevance  & Avg. \\
 \hline
Apex-PI-5 & 1.56 & 1.64 & 1.60 \\
Apex-PI-2 & \textbf{1.61} & 1.69 & \textbf{1.65}  \\
Apex-PI-1 & 1.56 & \textbf{1.72} & 1.64  \\
Apex-cost-anneal & 1.55 & 1.57 & 1.56 \\
Apex-cyclical-anneal  & 1.50 & 1.60  & 1.55 \\
Seq2seq & 1.55 & 1.57 & 1.56 \\
ExpansionNet  &1.56 & 1.50 & 1.53 \\
DP-GAN & 1.28 & 1.45 & 1.36 \\
 \hline
\end{tabular}\label{tab:human}
\end{table}

%%%----
Table~\ref{tab:human} illustrates the evaluation results by averaging the scores provided by graders. We can see that Apex-PI outperform the baselines in term of fluency and relevance. The fluency and relevance of Apex-PI-2 are better than those of Apex-PI-5. This is because a large KL divergence diversifies the generated text, but it lowers its quality. Besides, DP-GAN does not perform well because it is hard to stabilize the GAN. From this evaluation, we can conclude that KL divergence affects the accuracy of generated text. Thus, it is important to control the KL divergence to achieve the trade off between diversity and accuracy.


\begin{table*}\footnotesize
\centering
\caption{Generated text by different models with different order of input keywords. Case 1 and case 2 show that \textit{Apex} can totally control the order of keywords. Case2-1 and 2-2 show that \textit{Apex} can generate diverse text with the same order of input keywords. However, the baselines cannot control the order of keywords.}
\begin{tabular}{|m{3.5cm}|m{12cm}|}
\hline
\multicolumn{2}{|l|}{
\begin{CJK*}{UTF8}{gbsn}\footnotesize
Item: 半身裙~(skirt)
\end{CJK*}
}  \\ \hline
\multicolumn{2}{|l|}{
\begin{CJK*}{UTF8}{gbsn}\footnotesize
Input keywords: 撞色, 流苏, 迷人, 裙摆 ~(Contrasting color, Tassel, Charming/Charm, Skirt's hemline)
\end{CJK*}
} \\ \hline

\multicolumn{2}{|c|}{
\begin{CJK*}{UTF8}{gbsn}\footnotesize
Model: Apex-PI-2
\end{CJK*}
}  \\ \hline
%%--case 1--
\begin{CJK*}{UTF8}{gbsn}\footnotesize
Case 1: \newline
撞色(1), 流苏(2), 迷人(3),裙摆(4) \newline Contrasting color(1), Tassel(2), \newline Charming(3), Skirt's hemline(4)
\end{CJK*} & \begin{CJK*}{UTF8}{gbsn}\footnotesize
这款半身裙,采用了{\color{red}撞色流苏}的设计,丰富了裙身的细节,增添了几分灵动的气息,散发出 {\color{red}迷人}的气息.而{\color{red}裙摆}的流苏设计,更是增添了几分俏皮感,更显别致. \newline This skirt is designed with {\color{red}contrasting-color tassel}, which enriches its details, adds a bit of instant style and shows a {\color{red}charming} fashion. Plus, the {\color{red}skirt's hemline} is decorated with tassel, which makes it more playful and chic.
\end{CJK*} \\ \hline
%%---
\begin{CJK*}{UTF8}{gbsn}\footnotesize
Case 2-1 \newline
裙摆(1), 流苏(2), 迷人(3), 撞色(4) \newline Skirt's hemline(1), Tassel(2), \newline Charming(3), Contrasting color(4)
\end{CJK*} & \begin{CJK*}{UTF8}{gbsn}\footnotesize
{\color{red}裙摆}处的{\color{red}流苏}装饰,为整体增添了几分灵动的美感, 行走间摇曳出灵动的{\color{red}迷人}姿态.而裙身的{\color{red}撞色}线条, 则是将活力的气息展现的淋漓尽致, 让人看起来更加的与众不同. \newline The {\color{red}tassel} decoration on the {\color{red}skirt's hemline} adds a little of instant style, which helps people show a glamorous and {\color{red}charming} gesture when walking. Also, the {\color{red}contrasting color} of this skirt shows the vitality, making it out of the ordinary.
\end{CJK*}
\\ \hline
%%%case second
\begin{CJK*}{UTF8}{gbsn}\footnotesize
Case 2-2 (same as above) \newline
裙摆(1), 流苏(2), 迷人(3), 撞色(4) \newline Skirt's hemline(1), Tassel(2), \newline Charm(3), Contrasting color(4)
\end{CJK*}
& \begin{CJK*}{UTF8}{gbsn}\footnotesize
这款半身裙的{\color{red}裙摆}采用{\color{red}流苏}的设计,展现出一种灵动飘逸的美感,行走间展现出女性{\color{red}迷人}的魅力. 裙身{\color{red}撞色}的设计,丰富了视觉效果,展现出女性十足的青春活力,彰显出女性的个性与柔美. \newline
The {\color{red}skirt's hemline} is designed with {\color{red}tassel}, showing an instant style and {\color{red}charm} of ladies when walking. Its {\color{red}contrasting color} enriches the visual effects, fully showing the vitality and youth of women as well as their personality and beauty.
\end{CJK*}         \\ \hline

%% %%--case 2-3
% \begin{CJK*}{UTF8}{gbsn}\footnotesize
% Case 2-3 (same as above) \newline
% 裙摆(1), 流苏(2), 迷人(3), 撞色(4) \newline Skirt's hemline(1), Tassel(2), \newline Charming(3), Contrasting color(4)
% \end{CJK*}  &\begin{CJK*}{UTF8}{gbsn}\footnotesize
% {\color{red}裙摆}处的{\color{red}流苏}拼接,不仅增添了几分飘逸感,还散发出{\color{red}迷人}的气质. {\color{red}撞色}的腰带,不仅丰富了裙身的层次感,还能凸显出女性的曼妙身姿. \newline
% The {\color{red}tassel} decoration on the {\color{red}skirt's hemline} not only adds a bit of elegance, but also provides {\color{red}charming} feeling. The belt with {\color{red}contrasting color} not only improves a sense of layering of the skirt, but shows the elegant posture of ladies.
% \end{CJK*} \\ \hline
%%---seq2seq--
\multicolumn{2}{|c|}{Model: Seq2seq} \\ \hline
\begin{CJK*}{UTF8}{gbsn}\footnotesize
%Case 3: (unordered) \newline
撞色,迷人,裙摆,流苏\newline Tassel, Contrasting color, \newline Charming, Skirt's hemline
\end{CJK*}
& \begin{CJK*}{UTF8}{gbsn}\footnotesize
这款半身裙的亮点之处在于{\color{red}流苏}的设计,流苏的装饰,不仅展现出了与众不同的时尚品味,还增添了几分灵动的美感.而{\color{red}撞色}的格纹, 则展现出了一股复古的气息,彰显出了非凡的时尚品味,{\color{red}迷人}至极. \newline 
The fantastic part of this skirt is {\color{red}tassel}. With tassel as the decoration, the skirt not only shows distinctive fashion, but also provides a feeling of instant style. Moreover, its check pattern designed in {\color{red}contrasting color} shows vintage style and extraordinary fashion, which is very {\color{red}charming} and fantastic.
\end{CJK*}  \\ \hline
%% expansion
\multicolumn{2}{|c|}{Model: ExpansionNet} \\ \hline
 \begin{CJK*}{UTF8}{gbsn}\footnotesize
%Case 3: (unordered) \newline
撞色,迷人,裙摆,流苏 \newline
Tassel, Contrasting color, \newline Charming, Skirt's hemline
\end{CJK*} 
& \begin{CJK*}{UTF8}{gbsn}\footnotesize
上半身的{\color{red}流苏}带设计,让裙身的艺术感更加上升,同时整体的裙身上又展示出秀气利落之感,同时大摆裙的{\color{red}裙摆}行走间随风摇曳飘逸,行走间凸显潮流气息. \newline
The design of {\color{red}tassel} can improve the artistic sense of the skirt. The entire skirt also shows a sense of elegance. Moreover, the {\color{red}skirt's hemline} sways with the wind when the wearer is walking, making it looks more fashionable.
\end{CJK*}   \\ \hline
\multicolumn{2}{|c|}{Model: DP-GAN} \\ \hline
\begin{CJK*}{UTF8}{gbsn}\footnotesize
%Case 3: (unordered) \newline
撞色,迷人,裙摆,流苏 \newline
Tassel, Contrasting color, \newline Charming, Skirt's hemline
\end{CJK*}
& \begin{CJK*}{UTF8}{gbsn}\footnotesize
这质感的丝绒面料,让你在行走间散发出浪漫的气息.而裙身的{\color{red}撞色}设计,更是将女性的优雅气质展现的淋漓尽致.而裙身的{\color{red}流苏}装饰,则是以撞色的方式呈现出了一种独特的美感,让你在行走间散发出{\color{red}迷人}的气息. \newline 
This velvet fabric can make you send out a romantics taste. The design of {\color{red}contrasting color} on the skirt can totally show the elegance of ladies. In addition, its {\color{red}tassel} decoration shows a unique aesthetic feeling, making you look very {\color{red}charming} when walking.
\end{CJK*} \\ 
\hline
\end{tabular}\label{tab:control}
\end{table*}


%%%--case study---
\subsection{Case Study}
Finally, we do a case study to show \textit{Apex} can control the generated sentences based on the input keywords and their order customized by users. We shuffle the order of input keywords to generate different text.  Table~\ref{tab:control} illustrates an example of item descriptions generated by~\textit{Apex} and baselines\footnote{The order of keywords may be different in English translation}. For case 1 and case 2, we can see that our \textit{Apex} can totally control the orders of keywords in the generated text. For case 2-1 and 2-2, we use the same order of keywords to generate text. It can be seen that \textit{Apex} can generate diverse results with the same input order of keywords. However, the baseline methods sometimes miss some keywords in the generated text. Hence, \textit{Apex} outperforms the baselines in terms of diversity and accuracy. In addition, we show more examples in Appendix~\ref{app:example}.
